Calibrating Factual Knowledge in Pretrained Language Models

Previous literature has proved that Pretrained Language Models (PLMs) can store factual knowledge. However, we find that facts stored in the PLMs are not always correct. It motivates us to explore a fundamental question: How do we calibrate factual knowledge in PLMs without re-training from scratch? In this work, we propose a simple and lightweight method CaliNet to achieve this goal. To be specific, we first detect whether PLMs can learn the right facts via a contrastive score between right and fake facts. If not, we then use a lightweight method to add and adapt new parameters to specific factual texts. Experiments on the knowledge probing task show the calibration effectiveness and efficiency. In addition, through closed-book question answering, we find that the calibrated PLM possesses knowledge generalization ability after fine-tuning. Beyond the calibration performance, we further investigate and visualize the knowledge calibration mechanism.

==> EMNLP/040exp_v0.tex <==
\subsection{Wrong Factual Knowledge in PLMs}
We conduct CKA on 46 relations of TRE-X dataset. We first obtain the true relation pattern for each relation from LAMA, and manually write three false relation patterns for each relation. Then we sample 1000 facts for each relation and calculate CKA on each fact following Eq.~\ref{cka}, where $\mathbb{E}\left[P_M(o|s,r^{'})\right]$ is calculated as the mean probability of the three false relations.

The assessment result is shown in \qingxiu{todo: by relationship}.


Since CKA evaluates the model's knowledge of each fact, we identified the wrong knowledge in the PLM by CKA ($CKA_{M}(fact) < 5$). We statistically counted the wrong factual knowledge of T5 and it was found to account for XXX\% of all the facts, randomly sampled facts that T5 failed on are listed in Table ~\ref{table:detect}.

The results indicate that a high percentage of the knowledge stored in the model is incorrect. Therefore, it is urgent to correct the knowledge in PLMs.

\subsection{Calibration Ability}
\paragraph{Datasets}
Following the data construction process in Section ~\ref{data-construct}, we build paraphrased training and test sentences based on ParaREL~\cite{elazar2021measuring}
patterns. Except for the original test set with true entities, we create a false test via simply replacing the target entity with a false one.
To evaluate the general performance decline of the calibrated PLMs, we randomly mask the test data in the same manner as the that in the pretraining stage and name it C4 test. See Appendix ~\ref{}for details.

\paragraph{Metrics}
\qingxiu{todo: add CKA}
ppl
Rank-based


\subsubsection{Calibration Results}
\input{float/table-main}

Table ~\ref{table:main} reports the main results for
model calibration on factual knowledge. 
The calibration makes the model PPL decrease on True Test, and increase on False Test. That is, compared to the original model, our method adjusts the model to ``know'' about the given facts. In addition, our method has little effect on the model PPLon C4 Test because the model parameters are not destroyed like fine-tuning, thus retaining the semantic understanding ability. The EM and F1 of answer prediction further show that knowledge calibration enables the model to predict factual knowledge more accurately. The calibrated model no longer predicts high frequency or factually incorrect answers.

\subsubsection{Scalability Exploration}
To delve deeper into the scale of knowledge calibration, we implement our method on different scales of facts to be calibrated.

As Figure~\ref{fig:scale} illustrates, when the number of facts to be calibrated is small, the calibration F1 score is close to 100\%. As the number increases, the F1 score gradually decreases. When the number reaches 5000, our method still calibrates more than half of the facts for the PLM at once.
% A similar problem has been proposed and studied by ~\citet{roberts-etal-2020-much} in 2020. They directly take larger pretraining corpus as more knowledge and measure the amount of knowledge successfully packed into a PLM by the performance on downstream tasks like Natural Questions. While we restudy this problem, focus more on ``without external resourses, how much knowledge in a PLM can we calibrate at once''.

Compared to previous work on similar topics like model editing, the amount of knowledge that our method can calibrate at once is incredible. 
~\citet{mitchell2022fast} has proved that batched editing is difficult to change factual knowledge in PLMs. More concretely, when modifying more than 125 facts at one time, the success rate of model editing is less than 70\%. However, in our method, the success rate (EM) of calibrating more than 1000 facts is still greater than 70\%.

\input{float/figure-scale}


\subsubsection{Calibration Architecture Analysis}

\paragraph{How many calibration slots are needed?}

\input{float/table-dim}
As shown in Table~\ref{table:dim}, with a few calibration slots, both the EM score and the F1 score of knowledge calibration are low. While it is worth noting that, to calibrate 100 facts, only 64 calibration slots is sufficient to achieve the calibration effect equivalent to 3072 calibration slots. In terms of 1000 facts, 256 calibration slots are enough. We can conclude that when more facts are to be calibrated, the number of calibration slots needs to be appropriately increased. But in general, our method only takes a small number of parameters for calibration, mainly because our approach makes full use of the semantic modeling capabilities of the PLM itself. Therefore, the calibration only needs to adjust a small amount of wrong knowledge stored in the original model. 

\paragraph{Where to concatenate \resource{}?} 
As \resource{} is applicable to any FFN layer, we can concatenate it to any FFN layer in the Transformer. 
which layer
how many layers

\input{EMNLP/float/figure-layer}
Our FFN-expanding approach can generally be implemented on any model with a transformer architecture. As 


\subsection{Calibration Generalizability}
\paragraph{Datasets}
We validate the generalization ability of the calibrated knowledge in PLMs on three question answering datasets. The WebQuestions dataset~\cite{berant-etal-2013-semantic} is a question-answering dataset, including 6,642 QA pairs. The questions are created by crawling from Google Suggest API and the answers are obtained from crowdsourcing. All answers are entities.
The Natural Questions dataset~\cite{kwiatkowski2019natural} is a larger question answering dataset containing 307,373 training examples. Questions are queries aggregated from real users.  A short answer (one or more entities) is annotated for each question.

TriviaQA

\paragraph{Baselines} 
Pretrained LMs \\
Continual Pretrain \\

\input{EMNLP/float/table-wq}

==> EMNLP/040exp_v1.tex <==
\subsection{Knowledge Assessment and Calibration}
\input{EMNLP/float/figure-scale}
\input{EMNLP/float/table-dim}
\subsubsection{Datasets and Models} 
We sample various scales of factual triplets from the T-REx dataset~\cite{trex}. 
For each triplet, we fill its head and tail entities into the template in LAMA~\cite{lama} according to the relation. 
As a result, we construct datasets of varying sizes from 10 to 5000 natural sentences that express facts. 
We consider assessing and calibrating the factual knowledge in T5$_{\text{base}}$ and T5$_{\text{large}}$~\cite{t5} in our experiments.

\subsubsection{Metrics}
For knowledge assessment, we use both CKA and the rank-based assessment. 
For CKA, the smoothing factor is set to 0.001 and the threshold of false knowledge is set to 1 (i.e., we judge that the model does not store a correct fact if its CKA score is lower than 1). 
In rank-based assessment~\cite{lama}, we use Exact Match (EM) and F1 of the Top1 prediction.\footnote{Unlike LAMA, the length of our target entity is not limited, so we rank the predictions in an open vocabulary without picking out single-token entities.}
For knowledge calibration, our main evaluation metric is perplexity. 
Effective calibration increases the model perplexity on factually correct sentences and decreases the model perplexity on factually false sentences. 
We also calculate EM, F1 and CKA score for the calibrated PLMs.

\subsubsection{Detecting False Factual Knowledge}
\paragraph{Detection}
We utilize the CKA to detect false knowledge in T5.
For each relation in LAMA, we manually write $3$ erroneous relation templates. 
Then, for each fact, we fill the head entity into these templates to generate various negative probing prompts used in CKA. 
% We conduct CKA on 46 relations of TRE-X dataset. We first obtain the true relation pattern for each relation from LAMA, and manually write three pseudo relation patterns for each relation. 
After that, we calculate the CKA score for each fact following Equation~(\ref{cka}), where $\mathbb{E}\left[P_M(o|s,r^{'})\right]$ is computed by the average probability of the negative probing prompts.
Finally, we identify the false factual knowledge in the PLM whose CKA score is lower than 1. 

\paragraph{Results}
As shown in Table~\ref{table:main}, we find that the false facts accounts for nearly half of all the facts for T5-base. 
As for T5-large, which has a larger model capacity, its false rate is a little lower than T5-base but still quite high. 
The disappointingly high false rate in PLMs embodies the necessity to calibrate factual knowledge.

% \input{float/table-detect}
% We compare CKA score with the rank-based assessment used by previous work~\citep{lama} to show our advantages. 
% As shown in Table~\ref{table:detect}, the rank-based knowledge assessment suffers from inexhaustible answers and frequency bias.
% While in CKA, we evaluate each tail entity $o$ independently, so we no longer need to know all the other valid objects. In addition, $s$ appears in both the numerator and the denominator of CKA score, which neutralizes the influence of the frequency bias.
% % In short, compared with the rank-based assessment, CKA is better at dealing with inexhaustible answers and frequency bias so it can detect erroneous knowledge in PLMs more accurately. 

% In our experiments, we identify the false knowledge in the PLM by CKA score (CKA$_{\text{M}}$(fact) < 1). We statistically count the false factual knowledge of T5-base and find that it accounts for nearly half of all the facts; the assessment result is shown in Table~\ref{table:main}. Results indicate that a high percentage of the knowledge stored in the model is false. Therefore, it is necessary to correct the knowledge in PLMs.

\subsubsection{Calibrating False Factual Knowledge}

\paragraph{Settings}
The \resource{} consists of 64 and 256 calibration memory slots for 100 and 1000 target facts, respectively. 
Except for the original test set with correct facts, we also create an adversarial test set by replacing the target entity with a false one in the same entity type.
To verify the effect of calibration, we calculate the model perplexity before and after calibration on both test sets. 
In order to evaluate the general performance decline of the calibrated PLMs, we randomly mask the test data in the same manner as the that in the pretraining stage and denote it as general test set.
% See Appendix ~\ref{}for details.
Following ~\citet{continue}, we continue pretraining on the calibration data above as a baseline.

\paragraph{Results}
We show the results for knowledge calibration in Table~\ref{table:main}.  
The calibration makes the model perplexity decrease on the original test set, and increase on the adversarial test set. That is, compared to the original model, our method adjusts the model to ``know'' about the given facts. In addition, our method has little effect on the model perplexity on general test set because the model parameters are not destroyed like fine-tuning, thus its semantic understanding ability is well-retained.

We also assess the knowledge correctness of the calibrated model.
The improvement of Top1 prediction EM and F1 indicates that knowledge calibration enables the model to generate factually correct predictions. The overall false rate calculated via CKA score decreases from 48.10\% to 17.09\%, which further validates the effectiveness of the \resource{}.

\subsubsection{Scalability Exploration}
To delve deeper into the scale limitation of knowledge calibration, we implement our method on different scales of facts to be calibrated.

As Figure~\ref{fig:scale} illustrates, when the number of facts to be calibrated is small, the calibration F1 score is close to 100\%. As the number increases, the F1 score gradually decreases. When the number reaches 5000, our method still calibrates more than half of the facts in PLMs at once.
% A similar problem has been proposed and studied by ~\citet{roberts-etal-2020-much} in 2020. They directly take larger pretraining corpus as more knowledge and measure the amount of knowledge successfully packed into a PLM by the performance on downstream tasks like Natural Questions. While we restudy this problem, focus more on ``without external resourses, how much knowledge in a PLM can we calibrate at once''.

Compared to previous work on similar topics like knowledge editing (refer to Section~\ref{editing}), the amount of knowledge that \resource{} can calibrate at once is incredible. 
~\citet{mitchell2022fast} has proved that batched editing is difficult to change factual knowledge in PLMs. More concretely, when modifying more than 125 facts at one time, the success rate of model editing is less than 70\%. However, in our method, the EM improvement of calibrating more than 1000 facts is still greater than 70\%.

\subsubsection{Architecture Exploration}

\paragraph{How many calibration memory slots are needed?}


We run the experiments with different calibration memory slots and show the result in Table~\ref{table:dim}. To calibrate 100 facts, only 64 calibration memory slots is sufficient to achieve the calibration effect equivalent to 3072 calibration memory slots. In terms of 1000 facts, 256 calibration memory slots are enough. In addition, when more facts are to be calibrated, the number of calibration memory slots needs to be appropriately increased. In general, our method only takes a small number of parameters for calibration, mainly because our approach makes full use of the semantic modeling capabilities of the PLM itself. Therefore, the calibration only needs to adjust a small amount of false knowledge stored in the original model. 

\paragraph{Where to concatenate \resource{}?} 
As \resource{} is applicable to any FFN layer, we can concatenate it to any FFN layer in the Transformer and study the calibration ability of different layers.

Figure ~\ref{fig:layer} shows that deeper layers maintain stronger calibration ability. We suspect this is because the last two layers make full use of the semantic modeling capability of the previous layers. And if calibration is done in shallow layer, the adjusted hidden states may still be interfered by the false knowledge in the later FFNs.

\subsection{Calibration Generalizability}
\input{EMNLP/float/figure-layer}
\input{EMNLP/float/table-wq}


We validate the generalization ability of the calibrated knowledge in PLMs on WebQuestions~\cite{berant-etal-2013-semantic} and TriviaQA~\cite{tqa}. 

We fine-tune the PLM on the QA dataset without external knowledge bases. In this stage, the model learned to answer questions and only obtain related knowledge from the PLM (or some data overlap in the training data\cite{qaoverlap,canplm}). According to their prediction correctness on the test set, we aggregate the questions that
PLM answers incorrectly through its internal knowledge. Then, we retrieve all the triplets which include any entity in these questions from T-REx. Applying the method mentioned in Section~\ref{data-construct}, we transform the triplets for paraphrased natural sentences for \resource{} training. According to the facts to be calibrated, 64 calibration memory slots are trained for WebQuestions and 256 calibration memory sltos are trained for TriviaQA.
The calibrated PLM can be further fine-tuned on the question answering tasks. Our baseline is continue pretraining with our knowledge calibration data, the training objective of continue pretraining is restoring the masked entity and the model will also be finetuned on WebQuestions and TriaviaQA.
Our hyperparameter settings follows \citet{howmuch}.

The results are demonstrated in Table~\ref{table:wq}. On the one hand, model performance improves on the calibration subset, whose relative knowledge are calibrated through the approach we proposed. It indicates that the calibrated knowledge in PLMs can generalized to the downstream tasks. 
In addition, EM and F1 on the remaining questions are hardly impacted.
With only a few calibration memory slots, our method achieves the comparable knowledge calibration effect as continuing pretraining on all the parameters. According to the results in Table \ref{table:main}, continuing pre-training will affect the language modeling ability of PLMs. In contrast, our approach preserves the parameters of the original model well.

While on the other hand, the improvement on question answering is not large, which indicates that it is a difficult problem to fully use the correct knowledge in PLMs on the downstream tasks.


==> EMNLP/070impact.tex <==
Scientific work published at EMNLP 2022 must comply with the \href{https://www.aclweb.org/portal/content/acl-code-ethics}{ACL Ethics Policy}. We encourage all authors to include an explicit ethics statement on the broader impact of the work or other ethical considerations after the conclusion but before the references. The ethics statement will not count toward the page limit (8 pages for long, 4 pages for short papers).

==> EMNLP/float/table-scale.tex <==
\begin{table}[t]
\centering
    \begin{tabular}{rcccccccccc}
    \toprule
    \multirow{2}{*}{\bf Dim} &
    \multicolumn{2}{c}{100 facts} & 
    \multicolumn{2}{c}{1000 facts} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5}
    ~ &  EM & F1 & EM  &F1 \\
    \midrule
     10 & 0.0  & 0.0  & \bf 0.0 \\
     100 & 0.0   & 0.0 & \bf 0.0 \\
     1000 & 0.0  & 0.0 & \bf 0.0 \\
     10000 & 0.0 & 0.0 & \bf 0.0 \\
     \midrule
     \textbf{Avg} & 0.0 & 0.0 & \bf 0.0 \\
    \bottomrule
    \end{tabular}
\caption{Calibration ability with different numbers of calibration memory slots.}\label{table:scale}
\end{table}
